Phasebook: A Survey of Selected Open Problems in Phase Retrieval

Phase retrieval is an inverse problem that, on one hand, is crucial in many applications across imaging and physics, and, on the other hand, leads to deep research questions in theoretical signal processing and applied harmonic analysis. This survey paper is an outcome of the recent workshop Phase Retrieval in Mathematics and Applications (PRiMA) (held on August 5--9 2024 at the Lorentz Center in Leiden, The Netherlands) that brought together experts working on theoretical and practical aspects of the phase retrieval problem with the purpose to formulate and explore essential open problems in the field.

==> discussion.tex <==
% In case there will be a discussion, the last two lines of the introduction should be adapted.
%
%\section{Discussion}
%\label{S:Discussion}
